Efficient Sample-optimal Learning of Gaussian Tree Models via Sample-optimal Testing of Gaussian Mutual Information

Learning high-dimensional distributions is a significant challenge in machine learning and statistics. Classical research has mostly concentrated on asymptotic analysis of such data under suitable assumptions. While existing works [Bhattacharyya et al.: SICOMP 2023, Daskalakis et al.: STOC 2021, Choo et al.: ALT 2024] focus on discrete distributions, the current work addresses the tree structure learning problem for Gaussian distributions, providing efficient algorithms with solid theoretical guarantees. This is crucial as real-world distributions are often continuous and differ from the discrete scenarios studied in prior works. In this work, we design a conditional mutual information tester for Gaussian random variables that can test whether two Gaussian random variables are independent, or their conditional mutual information is at least $\varepsilon$, for some parameter $\varepsilon \in (0,1)$ using $\mathcal{O}(\varepsilon^{-1})$ samples which we show to be near-optimal. In contrast, an additive estimation would require $\Omega(\varepsilon^{-2})$ samples. Our upper bound technique uses linear regression on a pair of suitably transformed random variables. Importantly, we show that the chain rule of conditional mutual information continues to hold for the estimated (conditional) mutual information. As an application of such a mutual information tester, we give an efficient $\varepsilon$-approximate structure-learning algorithm for an $n$-variate Gaussian tree model that takes $\widetilde{\Theta}(n\varepsilon^{-1})$ samples which we again show to be near-optimal. In contrast, when the underlying Gaussian model is not known to be tree-structured, we show that $\widetilde{{{\Theta}}}(n^2\varepsilon^{-2})$ samples are necessary and sufficient to output an $\varepsilon$-approximate tree structure. We perform extensive experiments that corroborate our theoretical convergence bounds.

==> experiment.tex <==
\section{Experimental results}\label{sec:experiments}
In this section, we will present our experimental results. In \Cref{sec:experiment:chowliu}, we will present our results on Gaussian Chow-Liu where we compare the tolerance parameter ($\eps$) and the number of samples ($m$), along with linear regression plots for comparing $\log m$ vs $\log 1/\eps$. In particular, in \Cref{sec:experiment:chowliu:realizable}, we demonstrate our result on the realizable setting, and in \Cref{sec:experiment:chowliu:nonrealizable},we present our results for the non-realizable setting. Later in \Cref{sec:experiment:chowliuglasso}, we compare the Gaussian Chow-Liu result with Graphical Lasso (GLASSO), another method widely used in practice. We compare these two methods for $4$ settings of the tolerance parameter $\eps$. Finally in \Cref{sec:experiment:mitest}, we discuss our results on Mutual Information testing, where in \Cref{sec:experiment:mitest:realizable}, we study the realizable case, and in \Cref{sec:experiment:mitest:nonrealizable}, we present our results for additive estimation of mutual information.


\subsection{Experimental Setup}

%\color{blue}


\paragraph{Environment and Dataset} 
All experiments are carried out on a personal computer Mac Book Air with an M2 chip having a RAM of 8GB. All the experiments are conducted using synthetic datasets constructed using our hard constructions from the lower bound theorems. Experiments took a couple of hours at the most.

\color{black}

\subsection{Chow-Liu : $\eps$ vs $m^*$}\label{sec:experiment:chowliu}

In this experiment, we investigate the relationship between the number of samples required and the desired level of tolerance ($\eps$) for the Kullback-Leibler (KL) divergence to converge to zero. Specifically, we aim to determine the minimum number of samples necessary for the KL divergence between the original structure distribution and the predicted tree distribution to approach zero within a fixed tolerance $\varepsilon$.

\subsubsection{Realizable case}\label{sec:experiment:chowliu:realizable}

Let $U_1, V_1, W_1 \sim N(0,1)$ be three iid bits. Then, the realizable tree $R_1$ is defined as follows:
\begin{align*}
    Y_1  & \gets U_1\\
    Z_1  & \gets 0.5Y_1 + W_1 \\
    X_1 & \gets \sqrt{\eps} Z_1 + V_1
\end{align*}

For the fixing of tolerance ($\eps$), we are looking at the minimum number of samples($m$) at which the KL-Divergence between the original tree and the predicted tree using Chow-Liu algorithm is less than or equal to $\frac{\eps}{4}$ with probability $\geq 0.95$. Here, we are considering 1000 trials for every fixing of $\eps$. Then, note the least value of $m$ (i.e. $m^*$) for which the KL between predicted tree distribution and original tree distribution is less than or equal to $\frac{\eps}{4}$.

The relation between $m^*$ and $\eps$ for the realizable case with tree structure $R_1$ is as follows:

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/cl_r.png}
%     \caption{Proximity parameter vs No. of samples for the realizable case}
%     \label{fig:m_vs_eps}
% \end{figure}

After fitting the linear regression to the $\log(m^*)$ vs $\log\left(\frac{1}{\eps}\right)$ data, we obtain a line with a slope of $1.016$. $m^*$ is approximately inversely proportional to $\eps$.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/cl_r2.png}
%     \caption{$\eps$ vs $m^*$ linear regression for realizable case }
%     \label{fig:m_vs_eps}
% \end{figure}

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
     \includegraphics[width=0.8\linewidth]{Pics/cl_r.png}
        \caption{Proximity parameter vs No. of samples for the realizable case}
        \label{fig:prob1_6_2_realizable}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
    \includegraphics[width=0.8\linewidth]{Pics/cl_r2.png}
        \caption{$\eps$ vs $m^*$ linear regression for realizable case }
        \label{fig:prob1_6_1_realizable}
    \end{minipage}
\end{figure}


\pagebreak
\subsubsection{Non-realizable case}\label{sec:experiment:chowliu:nonrealizable}

Let us assume $B_1, U_1, V_1, W_1 \sim N(0,1)$ be four iid random bits. Then, the non-realizable structure $R_2$ is defined as follows:
\begin{align*}
 X_1 & \gets \paren{1+ \eps} \cdot B_1 + U_1 \\
 Y_1 & \gets \paren{1+ 2\eps} \cdot B_1 + V_1 \\
 Z_1  & \gets \paren{1+ 3\eps} \cdot B_1 + W_1
\end{align*}

For the fixing of tolerance ($\eps$), we are looking at the minimum number of samples ($m$) at which the KL-Divergence between the original graph and the predicted tree using the Chow-Liu algorithm is less than or equal to $\frac{\eps}{4}$ with probability $\geq 0.95$. Here, we are considering 1000 trials for every fixing of $\eps$. Then, noting the least value of $m$ (i.e.$m^*$) for which the KL between predicted tree distribution and original structure distribution is less than or equal to $\frac{\eps}{4}$.

% \begin{figure}[h]
%     \centering
%      \includegraphics[width=0.7\textwidth]{arxiv/Pics/cl_nr.png}
%     \caption{Proximity parameter vs No. of samples for the non-realizable case}
%     \label{fig:m_vs_eps_nr}
% \end{figure}

% \pagebreak

After fitting the linear regression to the $\log(m^*)$ vs $\log\left(\frac{1}{\eps}\right)$ data, we obtain a line with a slope of $1.916$. $m^*$ is approximately inversely proportional to $\eps^2$. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/cl_nr2.png}
%     \caption{$\eps$ vs $m^*$ linear regression for non-realizable case }
%     \label{fig:m_vs_eps}
% \end{figure}
% \pagebreak

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
     \includegraphics[width=0.8\linewidth]{Pics/cl_nr.png}
        \caption{Proximity parameter vs No. of samples for the non-realizable case}
        \label{fig:prob1_6_2_non_realizable}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
    \includegraphics[width=0.8\linewidth]{Pics/cl_nr2.png}
        \caption{$\eps$ vs $m^*$ linear regression for non-realizable case}
        \label{fig:prob1_6_1_non_realizable}
    \end{minipage}
\end{figure}


\subsection{Chow-Liu and GLASSO Comparison}\label{sec:experiment:chowliuglasso}

In this subsection, we compare the results of our Gaussian Chow-Liu algorithm with GLASSO, a popular algorithm used in the literature for estimation of covariance matrices.

\subsubsection{GLASSO}
The graphical lasso (GLASSO) is an algorithm for estimating sparse inverse covariance matrices in Gaussian graphical models, especially useful for high-dimensional data where the number of variables \( p \) exceeds the number of observations \( n \). It estimates the precision matrix \( \Theta = \Sigma^{-1} \), revealing conditional dependencies between variables.
The precision matrix \( \Theta \) is estimated by solving the optimization problem cited in \cite{friedman2008sparse}:

\[
\hat{\Theta} = \underset{\Theta \succ 0}{\text{argmin}} \left\{ \text{tr}(S \Theta) - \log \det(\Theta) + \lambda \|\Theta\|_1 \right\}
\]

Here, \( S \) is the sample covariance matrix, \( \|\Theta\|_1 \) is the element-wise \( \ell_1 \)-norm of \( \Theta \), and \( \lambda \) is a regularization parameter controlling sparsity. The \(\ell_1\)-penalty induces sparsity in \( \Theta \).

\subsubsection{Comparison experiments}
Firstly, we will set the original tree construction similar to \Cref{sec:experiment:chowliu}.

Let $U, V, W \sim N(0,1)$ be three iid bits. Then, the realizable tree $R_1$ is defined as follows:
\begin{align*}
    Y  & \gets U\\
    Z  & \gets 0.5Y + W \\
    X & \gets \sqrt{\eps} Z + V
\end{align*}

Then, do the following experiment on it.
We used the GLASSO package from R for the experiments~\cite{glassopackage}.
GLASSO returns a precision matrix for the triangle graph with the nodes $X,Y,Z$. We simply remove the lowest entry of the returned precision matrix in absolute value to obtain the approximate tree structure and compare the latter with the Chow-Liu output.
We conduct 200 trials to ascertain the frequency of correct recovery for various combinations of fixed epsilon and sample size ($m$). This gives us a way to compare the performance of the two algorithms to determine which requires fewer samples to prefer the $X$-$Z$ edge over the $X$-$Y$ edge.
We report this frequency of correct recovery in \Cref{fig:prob1_6_1_glasso_1}--\Cref{fig:prob1_6_4_glasso_4} by the above two algorithms for
100 different fixings of samples for $4$ different values of $\eps: 0.1,0.01,0.001,0.0001$.

% For $\eps = 0.0001$, the plot is as follows : 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/e_0.0001.png}
%     \caption{Chow-Liu vs Glasso for $\eps = 0.0001$}
%     \label{fig:m_vs_eps}
% \end{figure}
% \pagebreak


% For $\eps = 0.001$, the plot is as follows : 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/e_0.001.png}
%     \caption{Chow-Liu vs Glasso for $\eps = 0.001$}
%     \label{fig:m_vs_eps}
% \end{figure}

% \pagebreak


% For $\eps = 0.01$, the plot is as follows :

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/e_0.01.png}
%     \caption{Chow-Liu vs Glasso for $\eps = 0.01$}
%     \label{fig:m_vs_eps}
% \end{figure}
% \pagebreak

% For $\eps = 0.1$, the plot is as follows : 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/e_0.1.png}
%     \caption{Chow-Liu vs Glasso for $\eps = 0.1$}
%     \label{fig:m_vs_eps}
% \end{figure}
% \pagebreak

\begin{figure}
    \centering
    \begin{minipage}{.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Pics/e_0.1.png}
        \caption{Chow-Liu vs GLASSO for $\eps = 0.1$}
        \label{fig:prob1_6_1_glasso_1}
    \end{minipage}
    \begin{minipage}{.45\textwidth}
        \centering     \includegraphics[width=\linewidth]{Pics/e_0.01.png}
        \caption{Chow-Liu vs GLASSO for $\eps = 0.01$}
        \label{fig:prob1_6_2_glasso_2}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
        \centering
    \includegraphics[width=\linewidth]{Pics/e_0.001.png}
        \caption{Chow-Liu vs GLASSO for $\eps = 0.001$}
        \label{fig:prob1_6_3_glasso_3}
    \end{minipage}
    \begin{minipage}{.45\textwidth}
        \centering
     \includegraphics[width=\linewidth]{Pics/e_0.0001.png}
        \caption{Chow-Liu vs GLASSO for $\eps = 0.0001$}
        \label{fig:prob1_6_4_glasso_4}
    \end{minipage}%
\end{figure}


Overall, we can conclude that, for the tree-structured distributions, the Chow-Liu algorithm performs better than the GLASSO algorithm in reconstructing the structure from the samples. 

\subsection{Chow-Liu vs. CLIME}

\subsubsection{CLIME}

\begin{figure}
    \centering
    \begin{minipage}{.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{clime1.png}
        \caption{Chow-Liu vs CLIME for $\eps = 0.1$}
        \label{fig:prob1_7_1_clime_1}
    \end{minipage}
    \begin{minipage}{.45\textwidth}
        \centering     \includegraphics[width=\linewidth]{clime2.png}
        \caption{Chow-Liu vs CLIME for $\eps = 0.01$}
        \label{fig:prob1_7_2_clime_2}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
        \centering
    \includegraphics[width=\linewidth]{clime3.png}
        \caption{Chow-Liu vs CLIME for $\eps = 0.001$}
        \label{fig:prob1_7_3_clime_3}
    \end{minipage}
    \begin{minipage}{.45\textwidth}
        \centering
     \includegraphics[width=\linewidth]{clime4.png}
        \caption{Chow-Liu vs CLIME for $\eps = 0.0001$}
        \label{fig:prob1_7_4_clime_4}
    \end{minipage}%
\end{figure}



\subsection{MI testing experiments}\label{sec:experiment:mitest}

In this subsection, we present our mutual information testing experiment results. We start with the realizable setting, then move to the additive estimation experiment.

\subsubsection{Realizable case}\label{sec:experiment:mitest:realizable}
Let us assume $U, V \sim N(0,1)$ be two iid random bits. Then, the realizable structure $R_1$ is defined as follows:
\begin{align*}
 X & \gets U \\
 Y & \gets V \\
\end{align*}

We conducted experiments to investigate the impact of varying sample sizes on empirical mutual information. For each fixed value of \( m \), we calculated the average empirical mutual information over 1000 trials. Subsequently, we performed a regression analysis to determine the slope of the linear regression line fitted to the relationship between \( \log(m) \) and \( \log(\text{MI}) \). Our observations indicate that the slope of this line is approximately \( -1.003 \).


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/mi_r.png}
%     \caption{MI testing for realizable case}
%     \label{fig:log(m)_vs_log(mi)}
% \end{figure}
% \pagebreak

\subsubsection{Additive estimation of MI}\label{sec:experiment:mitest:nonrealizable}

Let us assume $U, V \sim N(0,1)$ be two iid random bits. Then, the non-realizable structure $R_2$ is defined as follows:
\begin{align*}
 X & \gets U \\
 Y & \gets X + V \\
\end{align*}
We conducted experiments to investigate the impact of varying sample sizes on empirical mutual information. For each fixed value of \( m \), we calculated the average empirical mutual information over 100 trials. Subsequently, we performed a regression analysis to determine the slope of the linear regression line fitted to the relationship between \( \log(m) \) and \( \log(\text{MI}) \). Our observations indicate that the slope of this line is approximately \( -0.5214 \). However, it is not completely clear to us why the variance is high in this experiment.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\textwidth]{arxiv/Pics/mi_nr.png}
%     \caption{MI testing for non-realizable case}
%     \label{fig:log(m)_vs_log(mi)}
% \end{figure}


\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
     \includegraphics[width=\linewidth]{Pics/mi_r.png}
        \caption{MI testing for realizable case}
        \label{fig:log(m)_vs_log(mi)}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
    \includegraphics[width=\linewidth]{Pics/mi_nr.png}
        \caption{Additive estimation of MI}
        \label{fig:log(m)_vs_log(mi)_est}
    \end{minipage}
\end{figure}    


\subsection{CMI testing experiments}

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
     \includegraphics[width=\linewidth]{Pics/cmi_lin_reg_r.png}
        \caption{CMI testing for realizable case}
        \label{fig:log(m)_vs_log(mi)_cmi}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
    \includegraphics[width=\linewidth]{Pics/cmi_lin_reg_nr.png}
        \caption{Additive estimation of CMI}
        \label{fig:log(m)_vs_log(mi)_est_cmi}
    \end{minipage}
\end{figure}  



==> experiment_main_version.tex <==
\section{Experimental results}\label{sec:experiment_main}
In this section, we report our experimental findings for our mutual information tester and the Chow-Liu algorithm.

%hi
%I am trying to call you but its not ringing. can you please try to call me again?
For the conditional mutual information testing, we use the hard distribution from the lower bound given by Theorem~\ref{theo:mitestlbintro}. The experiments confirm the theoretical finding that the convergence rate of $\wh{I}(X;Y)$ to $I(X;Y)$ scales as $m^{-0.5}$ in general but scales as $m^{-1}$ when $I(X;Y)=0$, as a function of the number of samples $m$. See Figure~\ref{fig:log(m)_vs_log(cmi)_est_main}.

% \begin{figure}
%     \centering
%      \includegraphics[width=\linewidth]{Pics/cmi_lin_reg_r.png}
%         \caption{CMI testing for realizable case}
%         \label{fig:log(m)_vs_log(cmi)_main}
% \end{figure}

% \begin{figure}    
%         \centering
%     \includegraphics[width=\linewidth]{Pics/cmi_lin_reg_nr.png}
%         \caption{Additive estimation of CMI}
%         \label{fig:log(m)_vs_log(cmi)_est_main}
% \end{figure}  

\begin{figure}    
        \centering
    \includegraphics[width=\linewidth]{cmi_picture_new2.png}
        \caption{CMI testing for realizable \& non-realizable cases}
        \label{fig:log(m)_vs_log(cmi)_est_main}
\end{figure}  

For the Chow-Liu experiments, we fix the three node graph given by our realizable hard construction of Theorem~\ref{theo:treelearningrealizablelbintro}, for 4 different fixings of $\eps$. We record the count of correct structure recovery among 200 repetitions as the number of samples varies for our Chow-Liu algorithm as well as two other popular algorithms GLASSO and CLIME. 
The experiments show that Chow-Liu performs better than the other two algorithms. See Figure~\ref{fig:chow-li-glasso-clime}.
\begin{figure}    
        \centering
    \includegraphics[width=\linewidth]{chow_liu_glasso_clime.png}
        \caption{Chow-Liu vs GLASSO and CLIME for $\eps=0.0001$}
        \label{fig:chow-li-glasso-clime}
\end{figure}  
Due to space constraints, we defer further experimental details to the Appendix.

% In the Graphical Lasso (GLASSO) the objective is to solve the following convex program
% $$
% \max_{\Theta \succ 0} \log \det(\Theta)- \langle \widehat{\Sigma}, \Theta \rangle - \lambda ||\Theta||_1
% $$
% Here $\widehat{\Sigma}$ is the empirical covariance matrix and $||\Theta||_1$ is the $\ell_1$ norm of the matrix as a vector.
% On the other hand, the CLIME
% estimator solves the following linear program:
% $$\min_{\Theta} ||\Theta||_1 \mbox{ st. } ||\widehat{\Sigma}\Theta - I||_{\infty}  \leq \lambda$$
% These two methods are widely used in the literature for learning Gaussian Graphical models (\cite{friedman2008sparse,ravikumar2011high,meinshausen2006high,kelner2020learning} and the references therein).



==> organization_app.tex <==
\begin{center}
\Huge
    Supplementary Material
\end{center}

\vspace{20pt}


\paragraph{Organization} 
In this supplementary material, we will present the proofs of the lemmas and theorems of the main paper. We will start with an additional preliminaries section in \Cref{sec:prelim_app}, stating some additional definitions and results, that we will use in the proofs.

In \Cref{sec:nonzeromean}, we start by showing that all our testing results continue to work for arbitrary mean Gaussian random variables by presenting a reduction to the zero-mean setting. 
Then we present our proof of the additive estimator of mutual information between two Gaussian random variables (\Cref{cl:miestboundintro}) in \Cref{sec:addtivemiest}, which we also prove is tight. Then in \Cref{sec:miub}, we give the proof of our mutual information tester for two Gaussian random variables (\Cref{lem:miubintro}), followed by the proof of the conditional mutual information tester (\Cref{lem:cmiubintro}) in \Cref{sec:cmiub}. We prove the chain rule of empirical conditional mutual information (\Cref{lem:cmichainruleempintro}) in \Cref{sec:cmichainrule}.
In \Cref{sec:mitestlb}, we present our result of the tight lower bound of mutual information tester (\Cref{theo:mitestlbintro}).

Later, in \Cref{sec:structurelearnnonzeromean}, we show reductions which prove that our structure learning results continue to hold for non-zero-mean setting. In \Cref{sec:nonrealizable}, we prove our structure learning result for non-realizable setting (\Cref{theo:treelearningnonrealizableintro}),
followed by the lower bound in the non-realizable setting (\Cref{theo:treelearningnonrealizablelbintro}). Then, in \Cref{sec:nonrealizablelb}, we present the proof of our structure learning result for realizable setting (\Cref{theo:treelearningrealizableintro}), followed by the associated lower bound (\Cref{theo:treelearningrealizablelbintro}) in \Cref{sec:realizablelb}. 

Finally, in \Cref{sec:experiments_full}, we present our detailed experimental results.


%\ssnotes{Can you please have a look at this?}



%We start ...



==> realizable_lb_new.tex <==
\subsection{Realizable structure learning lower bound}\label{sec:realizablelb}

Now we prove the tightness of our result for the realizable structure learning problem.

\treelearningrealizablelb*
% \begin{theo}\label{theo:treelearningrealizablelb}
% Given sample access to an unknown tree-structured zero-mean Gaussian distribution $P$, with probability at least $1-\delta$, $\Omega(\frac{n}{\eps} \log \frac{n}{\delta})$ samples from $P$ are necessary to output an $\eps$-approximate tree $T$.   
% \end{theo}

Similar to the non-realizable lower bound, we will first prove the lower bound for $n=3$ nodes. Then we will extend it for $n=3 \ell$, for some positive integer $\ell$.

Let $B_1, B_2, U_1, V_1, W_1, U_2, V_2, W_2 \sim N(0,1)$ be eight iid bits. The first tree $R_1$ is defined as follows:
\begin{align*}
    Y_1  & \gets U_1\\
    Z_1  & \gets \paren{1-\gamma}Y_1 + W_1 \\
    X_1 & \gets \sqrt{\frac{\eps}{n}} Z_1 + V_1
\end{align*}


% \begin{itemize}
%     \item[(i)] $X_1 \gets N(0,1)$,
%     \item[(ii)] $Y_1 \gets N(0,1) + b_1$, and
%     \item[(iii)] $Z_1 \gets \sqrt{\eps} X_1 + N(0,1) + b_1$.
% \end{itemize}

The second tree $R_2$ is defined as follows:
\begin{align*}
    Y_2 & \gets U_2 \\
    Z_2 & \gets \paren{1-\gamma}Y_2 + W_2\\
    X_2 & \gets \sqrt{\frac{\eps}{n}} Y_2 + V_2\\
\end{align*}

% \begin{itemize}
%     \item[(i)] $X_2 \gets N(0,1)$,
%     \item[(ii)] $Y_2 \gets \sqrt{\eps} X_1 + N(0,1) + b_2$, and
%     \item[(iii)] $Z_2 \gets N(0,1) +b_2 $.
% \end{itemize}

We will set $\gamma=1/2$ henceforth for our lower bound construction. Now we have the following two claims.
\begin{cl}\label{cl:realizableklbound} Fix $\gamma=1/2$.
 \begin{itemize}
     \item[(i)] $\kl(R_1||R_2) = 5\eps/4n$. Similarly, $\kl(R_2||R_1) = 5\eps/4n$.
     \item[(ii)] $I(X_1;Z_1)- I(X_1;Y_1) \geq \eps/2n$ and $I(X_2;Y_2)- I(X_2;Z_2) \geq 2\eps/5n$. 
 \end{itemize}   
\end{cl}

\begin{proof}

Let us first consider the covariance matrix of $R_1$ as follows:

$$\Sigma_1 = 
\begin{bmatrix}
\frac{\eps}{n}\paren{1-\gamma}^2 + \frac{\eps}{n} + 1 & \sqrt{\frac{\eps}{n}}\paren{1-\gamma} & \sqrt{\frac{\eps}{n}}\paren{1-\gamma}^2 + \sqrt{\frac{\eps}{n}} \\
\sqrt{\frac{\eps}{n}}\paren{1-\gamma} & 1 & \paren{1-\gamma} \\
\sqrt{\frac{\eps}{n}}\paren{1-\gamma}^2 + \sqrt{\frac{\eps}{n}} & \paren{1-\gamma} & \paren{1-\gamma}^2 + 1 
\end{bmatrix}$$

$$\Sigma_2 = 
\begin{bmatrix}
\frac{\eps}{n}+1 & \sqrt{\frac{\eps}{n}} & \paren{1-\gamma}\sqrt{\frac{\eps}{n}} \\
\sqrt{\frac{\eps}{n}} & 1 & \paren{1-\gamma} \\
\paren{1-\gamma}\sqrt{\frac{\eps}{n}} & \paren{1-\gamma} & \paren{1-\gamma}^2 + 1 
\end{bmatrix}$$

Note that for $\gamma = 1/2 $ $\det(\Sigma_1)= \det(\Sigma_2)=1$.

\begin{itemize}
    \item[(i)] 


From \Cref{obs:klhellingerbounds}, we know the following:
\begin{equation}
\kl(R_1 || R_2) = \frac{1}{2} \left(\tr(\Sigma_2^{-1} \Sigma_1) -3 + \ln\paren{\frac{\det(\Sigma_2)}{\det(\Sigma_1)}}\right)
\end{equation}

%We know that $\det(\Sigma_1)=\det(\Sigma_2)=1$. Also, $\det(\frac{\Sigma_1 + \Sigma_2}{2})= \frac{2+ \eps}{2}$.

Putting the values of $\Sigma_1$ and $\Sigma_2$ from above, we have:
\begin{eqnarray*}
\kl(R_1 || R_2) = 5\eps/4n.   
\end{eqnarray*}

Similarly, we can also show that $\kl(R_2 || R_1) = 5\eps/4n$. This completes our proof.

\item[(ii)]
\begin{eqnarray*}
I(X_1;Z_1) &=&  \frac{1}{2} \log \paren{1 + \frac{5\eps}{4n}} \\
I(Y_1;Z_1)  &=& \frac{1}{2} \log \paren{\frac{5}{4}} \\%\\ &\approx& \Theta(1)   
I(X_1;Y_1) &=& \frac{1}{2} \log \paren{\frac{\frac{5\eps}{4n}+1}{\frac{\eps}{n}+1}}   
\end{eqnarray*}

 Similarly,

%\item[(iii)]
\begin{eqnarray*}
I(X_2;Z_2) &=&  \frac{1}{2} \log \paren{\frac{1+\frac{\eps}{n}}{1 + \frac{4\eps}{5n}}}  \\
I(Y_2;Z_2)  &=& \frac{1}{2} \log \paren{\frac{5}{4}} \\%\\ &\approx& \Theta(1)   \\
I(X_2;Y_2) &=& \frac{1}{2} \log \paren{\frac{\eps}{n} + 1}   
\end{eqnarray*}    

Thus,  from above, we can say that
\begin{eqnarray*}\label{eqn:realizalemidiff}
I(X_1;Z_1)- I(X_1;Y_1) &=& \frac{1}{2}\log\paren{\frac{\eps}{n}+1}, \qquad \text{ and }    \label{eqn:realizalemidiff2}\\
I(X_2;Y_2)- I(X_2;Z_2) &=& \frac{1}{2}\log\paren{\frac{4\eps}{5n}+1}    
\end{eqnarray*}
\end{itemize}
\end{proof}

Thus,  the true structure tree $R_1$ will be of the form $Y-Z-X$ and similarly, the true structured tree $R_2$ will be of the form $X-Y-Z$. Thus, the edge $Y-Z$ will be present in both $R_1$ and $R_2$, and either $X-Z$ or $X-Y$ will be present, depending on the tree. Equivalently, we can represent each tree $R_1$ or $R_2$ as a Boolean bit, indicating whether a particular edge (without loss of generality, assume the edge $X-Z$) is present. So, if the tree is $R_1$ we will set the bit $1$, and if the tree is $R_2$, we set the bit to $0$.

Now we will construct a collection $\mathcal{D}$ of distributions, each over $\mathbb{R}^{3n}$, by choosing $n$ building blocks independent of each other, each is either $R_1$ or $R_2$. Note that, from the construction, $\size{\mathcal{D}}=2^n$.
Now consider a subset of $\dfar \subset \mathcal{D}$ such that if we take any two distributions $D_1, D_2 \in \dfar$ such that $\mathsf{Ham}(D_1,D_2) \geq n/5$.

%For any $3$ node tree, without loss of generality say $R_1$, we fix some canonical ordering of the edges: $(X_1Y_1, Y_1Z_1, X_1Z_1)$. Note that once we fix an ordering on the edges, we can represent $R_1$ as a Boolean string in $\{0,1\}^3$, where the $i$-th bit is $1$ if that edge is present in the tree. In a similar fashion, we will encode each tree-structured distribution over $\{0,1\}^n$ as a $n$ bit Boolean string.

We will start with the following observation.

\begin{obs}
\begin{itemize}
    \item[(i)] $\size{\dfar}= 2^{\Theta(n)}$.

    \item[(ii)] Consider any two arbitrary distribution $D_1, D_2 \in \dfar$. Then $\kl(D_1||D_2) \leq 5\eps/4$. Similarly, $\kl(D_2||D_1) \leq 5\eps/4$.
\end{itemize}
\end{obs}

\begin{proof}

\begin{itemize}
    \item[(i)] This follows from coding theory: the Gilbert-Varshamov bound, see \citep[Section 4.2]{guruswami2012essential} for reference.

    \item[(ii)] Consider any two arbitrary distributions $D_1, D_2 \in \dfar$. Note that $D_1$ and $D_2$ differ in $n/2$ bits, that is, $D_1$ and $D_2$ are different in $n/2$ building blocks. Without loss of generality, let us assume that the last $n/2$ bits are different. Since the building blocks of the distributions in $\dfar$ are chosen to be either $R_1$ or $R_2$, independently with equal probability, we can write the following:
    \begin{eqnarray*}
     \kl(D_1||D_2) &\le & n\cdot \kl(R_1||R_2) \\
     %&=& \sum_{i=n/2}^n \kl(R_1||R_2) \\
     %&=& \sum_{i=n/2}^n \left(I(X_1;Z_1)- I(X_1;Y_1)\right) \\
     &\leq& n \cdot \frac{5\eps}{4n}~~~~~~~~~~~~~~~~~~~[\mbox{From \Cref{cl:realizableklbound}}]\\
     &=& 5\eps/4
    \end{eqnarray*}
    
\end{itemize}
   Similarly, we can also show that $\kl(D_2||D_1) \leq 5\eps/4$. 
\end{proof}


Now we are ready to apply Fano's inequality (\Cref{lem:fanoinequality}) to obtain the desired testing lower bound. By \Cref{lem:fanoinequality}, we can say that to test correctly with probability at least $9/10$, we need at least
$$\Omega\left(\frac{\log \size{\dfar}}{\max\{\kl(D_1||D_2), \kl(D_2||D_1)\}}\right)$$

Since $\size{\dfar}= 2^{\Theta(n)}$, and $\max\{\kl(D_1||D_2), \kl(D_2||D_1)\} \leq 5\eps/4$, we need $\Omega(\frac{n}{\eps})$ samples to correctly test with probability at least $9/10$.

%From coding-theoretic results, we know that $\size{\mathcal{D}_{\mathsf{far}}}= 2^{\Theta(n)}$.

% We also have the following observation.

% \begin{obs}
% Consider any two arbitrary distribution $D_1, D_2 \in \mathcal{D}_{\mathsf{far}}$. Then $D_{KL}(D_1||D_2) \leq \eps$.
% \end{obs}

% \begin{proof}
% From ??, we know that $D_{KL}(R_1||R_2) \leq \eps$. Since both $D_1$ and $D_2$ are constructed by independently choosing $\ell$ copies of either $R_1$ or $R_2$, $D_{KL}(D_1||D_2) \leq n \eps$.     
% \end{proof}





% \begin{obs}\label{obs:realizabletreebound}

% \begin{itemize}
%     \item[(i)] Any tree $T$ on $3$ vertices is not $0.2 \eps$-approximate to any of  $R_1, R_2$ and $R_3$.

%     \item[(ii)] Consider the three trees $R_1, R_2$ and $R_3$. Given samples from one distribution $R_i$ with $i \in [3]$, in order to distinguish one distribution $R_j$ with $j \neq i$ with probability at least $2/3$, $\Omega(1/\eps)$ samples are required.
    
% \end{itemize}

% \end{obs}

% \begin{proof}

% \begin{itemize}
%     \item[(i)] Consider the three trees on $3$ nodes: $T_1= Y-X-Z$, $T_2= X-Y-Z$ and $T_3= X-Z-Y$. Let $R_{1,T_1}$ be the closest $T_1$-structured distribution of $R$. We define the other distributions $R_{1,T_2}$ and $R_{1,T_3}$.

% Now consider the fact that $D_{KL}(R||R_{1,T_1})- D_{KL}(R||R_{1,T_2})= I(X_1;Y_1)- I(X_1,Z_1) \geq 0.2 \eps$. This implies that $D_{KL}(R||R_{1,T_1}) \geq 0.2 \eps$. Similar bounds also hold for $D_{KL}(R||R_{1,T_2})$ and $D_{KL}(R||R_{1,T_3})$.  
% \end{itemize}
    
% \end{proof}

%\ssnotes{Shall we restate it here?}
%\sgnotes{Ok, I have removed it.}

\begin{proof}[Proof of \Cref{theo:treelearningrealizablelbintro}]
We consider a random distribution $D\in \dfar$. Any algorithm that guesses $\wh{D}$ correctly with at least 9/10 probability requires $\Omega(n\eps^{-1})$ samples. For every $i \in [n]$, let $(X_i,Y_i,Z_i)$ be the random variables for the $i$-th block. We will show that any algorithm $\mathcal{A}$ that returns an $\eps/16$-approximate tree will be able to correctly guess the true tree and therefore would need $\Omega(n\eps^{-1})$ samples. 




To see this, suppose $\mathcal{A}$ returns a tree structure $\wh{T}$ whereas the true tree structure is $T$. Let $\wh{D}=\arg \min\limits_{\textrm{tree distributions }P \ \textrm{on } \widehat{T}} \kl(D||P)$. Firstly, without loss of generality, we can remove the edges from $\wh{T}$ which connect across different blocks. Note that our true distribution belongs to $\dfar$ and does not have any such cross edges. The above follows due to the fact that the blocks are independent of each other, hence the mutual information between the corresponding nodes is $0$, thereby, the weights of the every cross edges are $0$ as well.


Now consider the case when $\wh{T}$ excludes an edge $(Y_i,Z_i)$ for some block $i \in [n]$. In that case, $\kl(D||\wh{D}) \ge \kl(D_i||\wh{D}_i) = I(Y_i;Z_i) - \max\{I(X_i;Z_i), I(X_i;Y_i)\} \ge \Theta(1)$ and $\wh{D}$ is no longer $\eps/16$-close,
where $D_i$ denotes the marginal distribution of the $i$-th block of $D$. Henceforth, we will assume that $\wh{D}\in \mathcal{D}$ without loss of generality.

Our guess for the unknown distribution $D$ will be $$D'=\arg \min\limits_{P \in \dfar} \ham(\wh{D},P).$$ Let $T'$ be the tree structure for $D'$. Note that $\ham(\wh{D},D')\le n/20$ as, otherwise, $\kl(\wh{D}||D)> \frac{n}{20} \cdot \frac{5\eps}{4n}=\frac{\eps}{16}$, leading to a contradiction. Henceforth, we will assume $\ham(\wh{D},D')\le n/20$.

In that case, by our construction, $\ham(\wh{D},D'')\ge \frac{n}{5}-\frac{n}{20} \ge \frac{3n}{20}>\frac{n}{20}$ for every $D''\in \dfar$ such that $D'\neq D''$. Therefore, there is a unique distribution in $\dfar$, which is exactly $D$ (as otherwise $\wh{D}$ will be $15\eps/16$-far), that is $\frac{n}{20}$-close to $\wh{D}$ in Hamming distance. This will be our guess for the unknown random distribution.


Combining all the cases, we see that using any $\eps/16$-approximate structure learning algorithm, we can correctly guess the random distribution without requiring any further samples. Therefore, the claimed lower bound holds.
\end{proof}

